New security notions and feasibility results for authentication of quantum data

We give a new class of security definitions for authentication in the quantum setting. These definitions capture and strengthen existing definitions of security against quantum adversaries for both classical message authentication codes (MACs) and well as full quantum state authentication schemes. The main feature of our definitions is that they precisely characterize the effective behavior of any adversary when the authentication protocol accepts, including correlations with the key. Our definitions readily yield a host of desirable properties and interesting consequences; for example, our security definition for full quantum state authentication implies that the entire secret key can be re-used if the authentication protocol succeeds. Next, we present several protocols satisfying our security definitions. We show that the classical Wegman-Carter authentication scheme with 3-universal hashing is secure against superposition attacks, as well as adversaries with quantum side information. We then present conceptually simple constructions of full quantum state authentication. Finally, we prove a lifting theorem which shows that, as long as a protocol can securely authenticate the maximally entangled state, it can securely authenticate any state, even those that are entangled with the adversary. Thus, this shows that protocols satisfying a fairly weak form of authentication security automatically satisfy a stronger notion of security (in particular, the definition of Dupuis, et al (2012)).

==> forging.tex <==
In this section we show that our security definition of authentication schemes relative to a basis imply the classical security definition of authentication schemes -- namely, that the adversary, after having received the authenticated message state, cannot produce two distinct authenticated message-tag pairs with non-negligible probability. This property is called \textbf{unforgeability}. We will see that unforgeability follows very easily from our security definition.

Our model for signature forgery is the following. Let $(\auth,\ver)$ be an authentication scheme in the basis $\basis$. As discussed before \hnote{Haven't added this discussion yet}, without loss of generality we can assume that the initial message state is a pure state $\ket{\rho}^{\msgspace \advspace} = \sum_m \alpha_m \ket{m}^\msgspace \otimes \ket{\varphi_m}^\advspace$ where the $\ket{\varphi_m}$ are arbitary pure states held by the adversary. After signing, we have
$$
	\sigma^{\keyspace \authspace \advspace} = \Ex_k \ketbra{k}{k} \otimes \auth_k ( \rho^{\msgspace \advspace} ).
$$
The adversary applies some CPTP quantum operation $\attack$ on $\authspace \advspace$ and outputs a system on $\authspace_1 \authspace_2 \advspace$. The spaces $\authspace_1$ and $\authspace_2$ are both isomorphic to $\authspace$. Let the tampered state be denoted as
$$
	\wt{\sigma}^{\keyspace \authspace_1 \authspace_2 \advspace} = \Ex_k \ketbra{k}{k} \otimes \attack(\auth_k ( \rho^{\msgspace \advspace} )).
$$
We define the \textbf{probability of forgery by $\attack$ on input $\rho$} to be the probability that, upon measuring $\keyspace$ in the computational basis, $\authspace_1$ and $\authspace_2$ in the basis $\basis$, we obtain a key $k$ and two states $\ket{\sigma}$ and $\ket{\sigma'}$ such that $\ket{\sigma} \neq \ket{\sigma'}$ and $\ver_k \ket{\sigma} = \ket{\sigma}$ and $\ver_k \ket{\sigma'} = \ket{\sigma'}$ (i.e. these states are valid tagged messages). \hnote{Or whatever the right notion of verification accepting is...}

The next theorem shows that quantum-secure authentication schemes possess the unforgeability property. The idea of the proof is as follows: suppose that there was an authentication scheme $(\auth,\ver)$, an adversary $\attack$ and an initial message state $\rho^{\msgspace}$ such that $\attack$ on input $\rho$ could forge an authenticated message with non-negligible probability. Using the fact that the authentication scheme is secure, we can in fact find a fixed message $m \in \msgspace$ and another adversary $\what{\attack}$ such that $\what{\attack}$, given an authentication of message $m$, forges an authenticated message $\psi'$ where $\psi' \neq \psi_k(m)$ with non-negligible probability. The definition of secure authentication scheme easily implies this is impossible. 

\newcommand{\forge}{{\mathsf{ForgeCheck}}}
\newcommand{\meas}{{\mathcal{M}}}

\begin{theorem}
	Let $(\auth,\ver)$ be an authentication scheme that is $\eps$-secure relative to basis $\basis$. Let $\attack$ be a CPTP map representing an adversary's behavior on authenticated message states. Then for all initial message states $\rho^{\msgspace \advspace}$, the probability of forgery by $\attack$ on input $\rho$ is at most $3\eps$.
\end{theorem}
\begin{proof}
	Suppose for contradiction that the probability of forgery is at least $\delta = 3\eps$. Here we shall treat each $\ver_k$ as the projector $\sum_{m} \ketbra{\psi_k(m)}{\psi_k(m)}$ acting on $\authspace_1$ where $\auth_k \ket{m} = \ket{\psi_k(m)}$. Define the projector
	$$
		\ver = \sum_k \ketbra{k}{k} \otimes \ver_k.
	$$
	Furthermore, we shall define the projector $\ver_k^{\neq \psi} = \sum_{m' : \psi_k(m') \neq \psi} \ketbra{\psi_k(m')}{\psi_k(m')}$ that acts on $\authspace_2$. That is, this projector accepts valid tagged messages except for one corresponding to a fixed message $m$. Define 
	$$
		\forge = \sum_{k,\psi} \ketbra{k}{k} \otimes \ketbra{\psi}{\psi} \otimes \ver_k^{\neq \psi}
	$$
	acting on $\keyspace \authspace_1 \authspace_2$, where the $\ket{\psi}$ are basis vectors in $\basis$. Furthermore, define $\meas_\basis^{\authspace_1 \authspace_2}$ to be the quantum operation that measures $\authspace_1$ and $\authspace_2$ in the basis $\basis$. Then since the probability of forgery is at least $\delta$, we have that
	$$
		\left \| \forge \circ \ver \circ \meas^{\authspace_1 \authspace_2}_\basis  \circ \attack(\sigma^{\keyspace \authspace \advspace}) \right \|_1 \geq \delta
	$$
	where $\sigma^{\keyspace \authspace \advspace} = \auth(\rho^{\keyspace \msgspace \advspace})$. 
	
	Now, since $(\auth,\ver)$ is an $\eps$-secure authentication scheme relative to basis $\basis$, there exists an ideal adversary $\id \in \ideal_\basis$ such that 
	$
		\left \| \ver(\attack(\sigma^{\keyspace \authspace \advspace})) - 	\ver(\id(\sigma^{\keyspace \authspace \advspace})) \right \|_1 \leq \eps
	$. Since the trace distance is non-increasing under quantum operations, we have that
	$$
		\left \| \forge \circ \meas^{\authspace_1 \authspace_2}_\basis \circ \ver \circ \attack(\sigma^{\keyspace \authspace \advspace}) - 	\forge \circ \meas^{\authspace_1 \authspace_2}_\basis \circ \ver \circ \id(\sigma^{\keyspace \authspace \advspace}) \right \|_1 \leq \eps
	$$ 
	where we used that $\meas^{\authspace_1 \authspace_2}_\basis$ commutes with $\ver$. This implies that 
	$$
		\left \| \forge \circ \meas^{\authspace_1 \authspace_2}_\basis \circ \ver \circ \id(\sigma^{\keyspace \authspace \advspace}) \right \|_1 \geq \delta - \eps.
	$$
	By Proposition~\ref{prop:characterization}, without loss of generality the ideal adversary behaves as follows: there exists an isometry $U$ mapping $\authspace \advspace$ to $\authspace_1 \authspace_2 \advspace \advspace'$ such that
	$$
		U \ket{\psi}^\authspace \otimes \ket{\varphi}^\advspace = \ket{\psi}^{\authspace_1} \otimes \ket{\theta_\psi}^{\authspace_2 \advspace} \otimes \left ( \delta_\psi \ket{0} + \sqrt{1 - \delta_\psi^2} \ket{1} \right)^{\advspace'}
	$$
	where $\ket{\psi}$ is a state in $\authspace_1$ and $\ket{\theta_\psi}$ is a pure state in $\authspace_2 \advspace$ and the last qubit is a state in $\advspace'$. Then
	$$
		\id(\sigma^{\keyspace \authspace \advspace}) = \Tr_{\advspace'} \left ( \Pi^{(0)} U \sigma^{\keyspace \authspace \advspace} U^\dagger \Pi^{(0)} \right)
	$$
	where $\Pi^{(0)} = \ketbra{0}{0}^{\advspace'}$ is the projector onto the $0$ qubit in $\advspace'$. Thus 
	\begin{align}
		\delta - \eps &\leq \left \| \forge \circ \meas^{\authspace_1 \authspace_2}_\basis \circ \ver( \Pi^{(0)} U \sigma^{\keyspace \authspace \advspace} U^\dagger\Pi^{(0)} ) \right \|_1 \\
					&= \left \| \Pi^{(0)} (\forge \circ \meas^{\authspace_1 \authspace_2}_\basis \circ \ver( U \sigma^{\keyspace \authspace \advspace} U^\dagger )) \Pi^{(0)}\right \|_1 \\
					&\leq \left \| \forge \circ \meas^{\authspace_1 \authspace_2}_\basis \circ \ver( U \sigma^{\keyspace \authspace \advspace} U^\dagger ) \right \|_1
	\end{align}
	where in the first equality we used that $\Pi^{(0)}$ commutes with $\forge$, $\meas^{\authspace_1 \authspace_2}_\basis$, and $\ver$ (because it acts on $\advspace'$), and that the trace norm is non-decreasing under quantum operations. Now, we have that $ \sigma^{\keyspace \authspace \advspace} = \Ex_k \ketbra{k}{k} \otimes \ketbra{\sigma_k}{\sigma_k}^{\authspace \advspace}$ where for each $k$, the state $\ket{\sigma_k} = \sum_m \alpha_m \ket{\psi_k(m)} \otimes \ket{\varphi_m}$. Then
	\begin{align}
		U \ket{\sigma_k} = \sum_m \alpha_m \ket{\psi_k(m)} \otimes \ket{\theta_{\psi_k(m)}} \otimes \left ( \delta_{\psi_k(m)} \ket{0} + \sqrt{1 - \delta_{\psi_k(m)}^2} \ket{1} \right).
	\end{align}
	For notational convenience we will let $\ket{\eta_{k,m}} = \delta_{\psi_k(m)} \ket{0} + \sqrt{1 - \delta_{\psi_k(m)}^2} \ket{1}$. Clearly, $\ver(U \sigma_k U^\dagger) = U \sigma_k U^\dagger$, and we have that\hnote{The following assumes $\auth_k$ is an isometry.}
	\begin{align*}
		&\forge \circ \meas^{\authspace_1 \authspace_2}_\basis \circ \ver ( U \sigma^{\keyspace \authspace \advspace} U^\dagger ) \\
		&= \Ex_k \ketbra{k}{k} \otimes \sum_m |\alpha_m|^2 \ketbra{\psi_k(m)}{\psi_k(m)} \otimes \left [\ver^{\neq \psi_k(m)}_k \circ \meas^{\authspace_2}_\basis (\ketbra{\theta_{\psi_k(m)}}{\theta_{\psi_k(m)}} ) \right ]\otimes \ketbra{\eta_{k,m}}{\eta_{k,m}}
\end{align*}
	where $\meas^{\authspace_2}_\basis $ denotes the operation of measuring $\authspace_2$ in basis $\basis$. We get then that 
	\begin{align}
	\delta - \eps &\leq \Ex_{k,m} \left \| \ver^{\neq \psi_k(m)}_k \circ \meas^{\authspace_2}_\basis (\ketbra{\theta_{\psi_k(m)}}{\theta_{\psi_k(m)}} ) \right \|_1
	\label{eq:forge0}
	\end{align}
	where the expectation $\Ex_{k,m}$ denotes $\Ex_{k} \sum_m |\alpha_m|^2$. The quantity on the right hand side of~\eqref{eq:forge0} denotes the probability that sampling $k \in \keyspace$, a message $m$, and measuring $\ket{\theta_{\psi_k(m)}}$ in the basis $\basis$ yields a forged authenticated message that's distinct from $\psi_k(m)$. Since $m$ is independent of $k$, we can switch the expectations, and by averaging get that there exists a single $m$ such that
		\begin{align}
	\delta - \eps &\leq \Ex_k \left \| \ver^{\neq \psi_k(m)}_k \circ \meas^{\authspace_2}_\basis (\ketbra{\theta_{\psi_k(m)}}{\theta_{\psi_k(m)}} ) \right \|_1.
	\label{eq:forging}
	\end{align}
	Consider the following scenario: let $\ket{\what{\rho}}^{\msgspace} = \ket{m}$. After authenticating with key $k$, we have $\ket{\what{\sigma}_k}^{\authspace} = \ket{\psi_k(m)}$, so
	$$
	\what{\sigma}^{\keyspace \authspace} = \Ex_k \ketbra{k}{k} \otimes \ketbra{\psi_k(m)}{\psi_k(m)}.
	$$
	Consider the following adversary $\what{\attack}$, which acts on $\authspace$ and outputs registers $\authspace_2 \advspace \authspace_1$:
	$$
		\what{\attack}(\what{\sigma}^{\keyspace \authspace}) = \meas^{\authspace_2}_\basis ( \ketbra{\theta_{\psi_k(m)}}{\theta_{\psi_k(m)}} \otimes \ketbra{\psi_k(m)}{\psi_k(m)} ).
	$$
	Note that the registers $\authspace_2 \advspace$ have been swapped with $\authspace_1$ -- we treat the registers $\advspace \authspace_1$ as being held by the adversary, and $\authspace_2$ is forwarded to the verifier. By~\eqref{eq:forging}, the state $\what{\attack}(\what{\sigma}^{\keyspace \authspace})$ passes the verification procedure with probability at least $\delta - \eps$. Thus, since $(\auth,\ver)$ is an $\eps$-secure authentication scheme relative to basis $\basis$, we also know that $\ver \circ \what{\attack}(\what{\sigma}^{\keyspace \authspace \advspace})$ is $\eps$-close to some ideal attack $\what{\id} \in \ideal_\basis$ on the authenticated state $\what{\sigma}^{\keyspace \authspace}$. By definition of an ideal attack, measuring the $\authspace_2$ register of $\ver \circ \what{\id}(\what{\sigma}^{\keyspace \authspace})$ with basis $\basis$ will yield only $\ket{\psi_k(m)}$. On the other hand, by~\eqref{eq:forging} measuring the first $\authspace$ register of $\ver \circ \what{\attack}(\what{\sigma}^{\keyspace \authspace})$ will yield a forged $\psi'$ that's distinct from $\psi_k(m)$ with probability at least $\delta - 2\eps > 0$, which is a contradiction.
	

	
\end{proof}

==> qkd.tex <==

In this section, we show that an $\epsilon$-secure QMAC satisfying total authentication implies Quantum Key Distribution. Protocol is as follows:
\begin{enumerate}
\item Alice prepares maximally entangled state over 2$l$ qubits i.e. $\ket{\Phi_L}=\frac{1}{\sqrt{L}}\sum_{x\in L}\ket{xx}^{L_1L_2}$. Alice chooses key $k$ at random and authenticates $L_2$ using QMAC protocol. After authentication, let the state be $\sum_{x\in L}\ket{x\sigma_x}^{L_1\mathcal{Y}}$.
\item Alice sends $\mathcal{Y}$ part to Bob.
\item Bob sends a bit to Bob after he receives $\tau^\mathcal{Y}$ through the quantum channel.
\item Alice sends the key $k$ over a classical channel that can be intercepted by the same adversary for the quantum channel. 
\item Bob applies the Verification procedure on state $\tau^\mathcal{Y}$ to get a state in $L_2$. He sends bit $b$ to Alice representing if verifier accepted ($b=1$) or rejected.
\item If $b=1$, Alice measures qubits in $L_1$ and uses the final collapsed state $x$ as the secret key. If adversary had just forwarded the state that he received, after verification, qubits in $L_1$ and $L_2$ would be maximally entangled and thus Alice and Bob end up with same random $l$ bits.
\end{enumerate}
Alice and Bob repeat the above procedure $n$ times in parallel. \\
We have an $\epsilon$-secure QMAC implying \[||\mathbb{E}_{k}\ket{k}\bra{k}\otimes[(\text{Ver}_k\otimes \mathbb{I}^{\mathcal{Z}})\circ\mathcal{O}\circ(\text{Auth}_k\otimes \mathbb{I}^{\mathcal{Z}})(\rho^{\mathcal{MZ}})]-\mathbb{E}_{k}\ket{k}\bra{k}\otimes[(\text{Ver}_k\otimes \mathbb{I}^{\mathcal{Z}})\circ\mathcal{I}\circ(\text{Auth}_k\otimes \mathbb{I}^{\mathcal{Z}})(\rho^{\mathcal{MZ}})]||_1\le \epsilon\]
%Here, $\mathcal{O}$ and $\mathcal{I}$ are real and ideal adversaries respectively. 
Here, $L_2$ register corresponds to $M$ in the above equation. $\mathcal{I}$ is an oblivious adversary i.e. there exists a superoperator $\mathcal{S}$ acting on $\mathcal{Z}$ such that $\mathcal{I}=\mathbb{I}^\mathcal{Y}\otimes\mathcal{S}$. Security equation becomes
\[||\mathbb{E}_{k}\ket{k}\bra{k}\otimes[(\text{Ver}_k\otimes \mathbb{I}^{\mathcal{Z}})(\tau^{\mathcal{YZ}})]-\mathbb{E}_{k}\ket{k}\bra{k}\otimes[(\text{Ver}_k\otimes \mathbb{I}^{\mathcal{Z}})\circ(\mathbb{I}^\mathcal{Y}\otimes\mathcal{S})(\sigma^\mathcal{YZ})]||_1\le \epsilon\]
\[\implies \mathbb{E}_k||(\text{Ver}_k\otimes \mathbb{I}^{\mathcal{Z}})(\tau^{\mathcal{YZ}})-(\text{Ver}_k\otimes \mathbb{I}^{\mathcal{Z}})\circ(\mathbb{I}^\mathcal{Y}\otimes\mathcal{S})(\sigma^\mathcal{YZ})||_1\le\epsilon\]
Thus, with probability $\ge 1-\frac{1}{\lambda}$, Alice chooses a key such that \[||(\text{Ver}_k\otimes \mathbb{I}^{\mathcal{Z}})(\tau^{\mathcal{YZ}})-(\text{Ver}_k\otimes \mathbb{I}^{\mathcal{Z}})\circ(\mathbb{I}^\mathcal{Y}\otimes\mathcal{S})(\sigma^\mathcal{YZ})||_1\le\lambda\epsilon\]
An ideal adversary never touches the $\mathcal{Y}$ register and $\mathcal{S}$ is independent of $\mathcal{Y}$ and $k$. In the ideal case, adversary learns nothing about the key $k$ and the state, after acceptance, remains completely entangled with $L_1$ (acceptance probability depends on $\mathcal{S}$). As the trace distance for the state ($\mathcal{MZ}$) between two adversaries is not greater than $\lambda\epsilon$, \[\Pr[\text{Bob accepts and adversary learns something about the key $k$ or $x$}]\le \lambda\epsilon\] Alice and Bob use the entangled state only if Bob accepts. Repeating it $n$ times, we get that with probability higher that $1-n(\frac{1}{\lambda}+\lambda\epsilon)$, Alice and Bob have the same secret key of which adversary has no knowledge about. The size of the secret key depends on the adversary's attack frequency. We repeat it $n$ times to estimate this frequency.\\
Choosing $\lambda=\epsilon^{-1/2}$, we get probability of failure as $\le2n\sqrt{\epsilon}$.





